Tokenization Matters: Navigating Data-Scarce Tokenization for Gender Inclusive Language Technologies

Gender-inclusive NLP research has documented the harmful limitations of gender binary-centric large language models (LLM), such as the inability to correctly use gender-diverse English neopronouns (e.g., xe, zir, fae). While data scarcity is a known culprit, the precise mechanisms through which scarcity affects this behavior remain underexplored. We discover LLM misgendering is significantly influenced by Byte-Pair Encoding (BPE) tokenization, the tokenizer powering many popular LLMs. Unlike binary pronouns, BPE overfragments neopronouns, a direct consequence of data scarcity during tokenizer training. This disparate tokenization mirrors tokenizer limitations observed in multilingual and low-resource NLP, unlocking new misgendering mitigation strategies. We propose two techniques: (1) pronoun tokenization parity, a method to enforce consistent tokenization across gendered pronouns, and (2) utilizing pre-existing LLM pronoun knowledge to improve neopronoun proficiency. Our proposed methods outperform finetuning with standard BPE, improving neopronoun accuracy from 14.1% to 58.4%. Our paper is the first to link LLM misgendering to tokenization and deficient neopronoun grammar, indicating that LLMs unable to correctly treat neopronouns as pronouns are more prone to misgender.

==> tables/70m_exp.tex <==
\begin{table*}[h]
    \small
    \centering
    \renewcommand{\arraystretch}{1} % Adjust the spacing between rows
\setlength{\tabcolsep}{3pt} % Adjust the space between columns
\caption{70M-parameter model results at 10\% data resource level.  $T_{\text{Orig}}$= without \texttt{PTP}, $T_{\text{PTP}}$= with \texttt{PTP},  $M_{\text{Full}}$= full finetuning, $M_{\text{Lex}}$= only lexical finetuning. $M_{\text{Baseline}}$= original model, no finetuning. The uncertainty estimates are 95\% confidence intervals computed from 10k bootstrap iterations. }
\label{tbl:70m_model_comparison}
\begin{tabular}{l|ccc|ccc|ccc} 
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}}             & \multicolumn{3}{c|}{\textbf{Pronoun Consistency ($\uparrow$)}}                                                    & \multicolumn{3}{c|}{\textbf{Case Agreement ($\uparrow$)}}                                                          & \multicolumn{3}{c}{\textbf{Error ($\downarrow$)}}                                                                   \\
\multicolumn{1}{c|}{}                                            & \textbf{He}                          & \textbf{She}                         & \textbf{Xe}                         & \textbf{He}                          & \textbf{She}                         & \textbf{Xe}                          & \textbf{He}                          & \textbf{She}                         & \textbf{Xe}                           \\ 
\midrule
\graytext{$\text{T}_{\text{Orig}} + \text{M}_{\text{Baseline}}$} & \graytext{96.82\textsubscript{0.79}} & \graytext{71.59\textsubscript{2.00}} & \graytext{0.67\textsubscript{0.36}} & \graytext{67.69\textsubscript{2.10}} & \graytext{60.72\textsubscript{2.15}} & \graytext{20.00\textsubscript{1.77}} & \graytext{23.85\textsubscript{1.90}} & \graytext{16.92\textsubscript{1.67}} & \graytext{85.03\textsubscript{1.62}}  \\




$\text{T}_\text{Orig} + \text{M}_\text{Full}$                    & 89.64\textsubscript{1.36}            & 86.05\textsubscript{1.51}            & 14.46\textsubscript{1.56}           & 68.51\textsubscript{2.08}            & 59.69\textsubscript{2.21}            & 20.00\textsubscript{1.77}            & 23.95\textsubscript{1.87}            & 16.77\textsubscript{1.64}            & 89.49\textsubscript{1.38}             \\
$\text{T}_\text{PTP} + \text{M}_\text{Full}$                     & 94.77\textsubscript{1.00}            & 83.49\textsubscript{1.64}            & 37.79\textsubscript{2.15}           & 69.49\textsubscript{2.03}            & 61.08\textsubscript{2.18}            & 29.38\textsubscript{2.05}            & 27.79\textsubscript{1.97}            & 20.97\textsubscript{1.77}            & 27.03\textsubscript{1.97}             \\
\bottomrule
\end{tabular}
\label{tbl:70m_model_comparison}
\end{table*}




% \begin{table*}[h]
%     \small
%     \centering
%     \renewcommand{\arraystretch}{1} % Adjust the spacing between rows
% \setlength{\tabcolsep}{3pt} % Adjust the space between columns
%     \begin{tabular}{l|ccc|ccc|ccc} 
%     \toprule
%     \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{3}{c|}{\textbf{Pronoun Consistency ($\uparrow$)}} & \multicolumn{3}{c|}{\textbf{Case Agreement ($\uparrow$)}} & \multicolumn{3}{c}{\textbf{Error ($\downarrow$)}}                                                                                  \\
%              & \textbf{He} & \textbf{She} & \textbf{Xe} & \multicolumn{1}{c}{\textbf{He}} & \textbf{She} & \textbf{Xe} & \multicolumn{1}{c}{\textbf{He}} & \multicolumn{1}{c}{\textbf{She}} & \multicolumn{1}{c}{\textbf{Xe}} \\ 
%     \midrule
% \graytext{$\text{T}_{\text{Orig}}  + \text{M}_{\text{Baseline}}$}& \graytext{96.82\textsubscript{0.79}} & \graytext{71.59\textsubscript{2.00}} & \graytext{0.67\textsubscript{0.36}}&\graytext{67.69\textsubscript{2.10}}& \graytext{60.72\textsubscript{2.15}} & \graytext{20.00\textsubscript{1.77}}&\graytext{23.85\textsubscript{1.90}} & \graytext{16.92\textsubscript{1.67}} & \graytext{85.03\textsubscript{1.62}} \\ $\text{T}_{\text{Orig}} + \text{M}_{\text{Full}}$ &89.64\textsubscript{1.36} & 86.05\textsubscript{1.51} & 14.46\textsubscript{1.56}&68.51\textsubscript{2.08} & 59.69\textsubscript{2.21} & 20.00\textsubscript{1.77}&23.95\textsubscript{1.87} & 16.77\textsubscript{1.64} & 89.49\textsubscript{1.38} \\ $\text{T}_{\text{Orig}} + \text{M}_{\text{Lex}}$&86.46\textsubscript{1.54} & 72.87\textsubscript{1.97} & 16.77\textsubscript{1.67}&61.74\textsubscript{2.15} & 57.18\textsubscript{2.18} & 20.00\textsubscript{1.74}&28.97\textsubscript{1.97} & 23.18\textsubscript{1.87} & 65.44\textsubscript{2.10} \\ $\text{T}_{\text{PTP}} + \text{M}_{\text{Full}}$&94.77\textsubscript{1.00} & 83.49\textsubscript{1.64} & 37.79\textsubscript{2.15}&69.49\textsubscript{2.03} & 61.08\textsubscript{2.18} & 29.38\textsubscript{2.05}&27.79\textsubscript{1.97} & 20.97\textsubscript{1.77} & 27.03\textsubscript{1.97} \\ 

% % $\text{T}_{\text{PTP-B}} + \text{M}_{\text{Full}}$&96.21\textsubscript{0.85} & 80.72\textsubscript{1.77} & 24.36\textsubscript{1.90}&68.92\textsubscript{2.05} & 61.23\textsubscript{2.15} & 23.13\textsubscript{1.90}&28.26\textsubscript{1.97} & 20.56\textsubscript{1.79} & 25.95\textsubscript{1.95} \\ 

% $\text{T}_{\text{PTP}} + \text{M}_{\text{Lex}}$&84.97\textsubscript{1.56} & 72.21\textsubscript{1.95} & 53.59\textsubscript{2.18}&63.23\textsubscript{2.18} & 59.13\textsubscript{2.21} & 32.51\textsubscript{2.08}&25.79\textsubscript{1.92} & 21.85\textsubscript{1.82} & 34.77\textsubscript{2.13} \\ 

% % $\text{T}_{\text{PTP-B}} + \text{M}_{\text{Lex}}$&83.28\textsubscript{1.67} & 74.31\textsubscript{1.90} & 42.97\textsubscript{2.18}&65.44\textsubscript{2.13} & 59.64\textsubscript{2.15} & 33.23\textsubscript{2.08}&24.31\textsubscript{1.90} & 20.21\textsubscript{1.77} & 32.05\textsubscript{2.08} \\ 


%     \bottomrule
%     \end{tabular}
%     \captionof{table}{70M-parameter model results at 10\% data resource level.  $T_{\text{Orig}}$= without \texttt{PTP}, $T_{\text{PTP}}$= with \texttt{PTP},  $M_{\text{Full}}$= full finetuning, $M_{\text{Lex}}$= only lexical finetuning. $M_{\text{Baseline}}$= original model, no finetuning. The uncertainty estimates are 95\% confidence intervals computed from 10k bootstrap iterations. 
%     \label{tbl:70m_model_comparison}}
% \end{table*}




==> tables/benchmarks_all.tex <==
\begin{table*}
\renewcommand{\arraystretch}{0.7} % Adjust the horiztontal spacing
\setlength{\tabcolsep}{1pt} % Adjust the wdith space between columns
\tiny
\centering
\caption{table}
\label{tbl:70m_model_comparison}
% \begin{tabular}{llccccccccccc}
\begin{tabular}{lllllllllllll}
% \newcolumntype{C}{ @{}>{${}}c<{{}$}@{} }
% \begin{tabular}{ll *13{rCl} }
% \begin{tabular}{ll*{11}{>{$}r<{$}@{}>{$}l<{$}}>{$}l<{$}}
\toprule
Size & Version & arc-c & arc-e & hellaswag & lambada & logiqa & piqa & sciq & triviaqa & truthfulqa1 & truthfulqa2 & winogrande \\ 
\midrule
\multirow[t]{5}{*}{70m}& Baseline & $ 19.71 \pm 1.16 $ & $ 35.94 \pm 0.98 $ & $ 27.62 \pm 0.45 $ & $ 10.87 \pm 0.43 $ & $ 27.96 \pm 1.76 $ & $ 58.32 \pm 1.15 $ & $ 58.50 \pm 1.56 $ & $ 0.16 \pm 0.03 $ & $ 25.70 \pm 1.53 $ & $ 47.56 \pm 1.57 $ & $ 49.17 \pm 1.41 $\\ 
& $\text{T}_{\text{Orig}} + \text{M}_{\text{Full}}$ & $ 22.18 \pm 1.21 $ & $ 32.70 \pm 0.96 $ & $ 27.30 \pm 0.44 $ & $ 9.04 \pm 0.40 $ & $ 26.57 \pm 1.73 $ & $ 55.44 \pm 1.16 $ & $ 52.30 \pm 1.58 $ & $ 0.02 \pm 0.01 $ & $ 29.38 \pm 1.59 $ & $ 54.53 \pm 1.64 $ & $ 49.64 \pm 1.41 $\\ 
& $\text{T}_{\text{PTP}} + \text{M}_{\text{Baseline}}$ & $ 21.93 \pm 1.21 $ & $ 32.58 \pm 0.96 $ & $ 27.26 \pm 0.44 $ & $ 8.78 \pm 0.39 $ & $ 25.50 \pm 1.71 $ & $ 55.82 \pm 1.16 $ & $ 55.60 \pm 1.57 $ & $ 0.02 \pm 0.01 $ & $ 28.64 \pm 1.58 $ & $ 53.27 \pm 1.65 $ & $ 50.43 \pm 1.41 $\\ 
& $\text{T}_{\text{Orig}} + \text{M}_{\text{Lex}}$ & $ 23.72 \pm 1.24 $ & $ 30.01 \pm 0.94 $ & $ 27.46 \pm 0.45 $ & $ 9.40 \pm 0.41 $ & $ 29.03 \pm 1.78 $ & $ 50.00 \pm 1.17 $ & $ 51.80 \pm 1.58 $ & $ 0.01 \pm 0.01 $ & $ 31.82 \pm 1.63 $ & $ inf \pm inf $ & $ 50.51 \pm 1.41 $\\ 
& $\text{T}_{\text{PTP}} + \text{M}_{\text{Lex}}$ & $ 23.72 \pm 1.24 $ & $ 30.39 \pm 0.94 $ & $ 27.63 \pm 0.45 $ & $ 9.40 \pm 0.41 $ & $ 29.49 \pm 1.79 $ & $ 50.33 \pm 1.17 $ & $ 51.30 \pm 1.58 $ & $ 0.01 \pm 0.01 $ & $ 33.66 \pm 1.65 $ & $ inf \pm inf $ & $ 50.99 \pm 1.40 $\\ 
\midrule 
\multirow[t]{5}{*}{160m}& Baseline & $ 23.63 \pm 1.24 $ & $ 43.18 \pm 1.02 $ & $ 31.59 \pm 0.46 $ & $ 23.20 \pm 0.59 $ & $ 26.27 \pm 1.73 $ & $ 62.84 \pm 1.13 $ & $ 77.90 \pm 1.31 $ & $ 2.21 \pm 0.11 $ & $ 24.60 \pm 1.51 $ & $ 43.93 \pm 1.52 $ & $ 49.72 \pm 1.41 $\\ 
& $\text{T}_{\text{Orig}} + \text{M}_{\text{Full}}$ & $ 24.74 \pm 1.26 $ & $ 38.09 \pm 1.00 $ & $ 30.18 \pm 0.46 $ & $ 16.99 \pm 0.52 $ & $ 25.96 \pm 1.72 $ & $ 58.16 \pm 1.15 $ & $ 68.40 \pm 1.47 $ & $ 0.40 \pm 0.05 $ & $ 27.29 \pm 1.56 $ & $ 49.94 \pm 1.62 $ & $ 52.09 \pm 1.40 $\\ 
& $\text{T}_{\text{PTP}} + \text{M}_{\text{Baseline}}$ & $ 24.15 \pm 1.25 $ & $ 37.92 \pm 1.00 $ & $ 29.65 \pm 0.46 $ & $ 15.80 \pm 0.51 $ & $ 27.04 \pm 1.74 $ & $ 57.40 \pm 1.15 $ & $ 67.60 \pm 1.48 $ & $ 0.43 \pm 0.05 $ & $ 27.91 \pm 1.57 $ & $ 50.62 \pm 1.62 $ & $ 52.17 \pm 1.40 $\\ 
& $\text{T}_{\text{Orig}} + \text{M}_{\text{Lex}}$ & $ 24.49 \pm 1.26 $ & $ 35.14 \pm 0.98 $ & $ 29.05 \pm 0.45 $ & $ 15.31 \pm 0.50 $ & $ 29.80 \pm 1.79 $ & $ 53.21 \pm 1.16 $ & $ 71.00 \pm 1.44 $ & $ 0.38 \pm 0.05 $ & $ 29.62 \pm 1.60 $ & $ 51.78 \pm 1.63 $ & $ 48.38 \pm 1.40 $\\ 
& $\text{T}_{\text{PTP}} + \text{M}_{\text{Lex}}$ & $ 26.02 \pm 1.28 $ & $ 35.14 \pm 0.98 $ & $ 28.83 \pm 0.45 $ & $ 15.21 \pm 0.50 $ & $ 29.49 \pm 1.79 $ & $ 52.72 \pm 1.16 $ & $ 70.30 \pm 1.45 $ & $ 0.23 \pm 0.04 $ & $ 30.60 \pm 1.61 $ & $ 52.76 \pm 1.62 $ & $ 48.15 \pm 1.40 $\\ 
\midrule 
\multirow[t]{5}{*}{410m}& Baseline & $ 25.85 \pm 1.28 $ & $ 51.81 \pm 1.03 $ & $ 41.36 \pm 0.49 $ & $ 39.32 \pm 0.68 $ & $ 24.12 \pm 1.68 $ & $ 67.52 \pm 1.09 $ & $ 87.70 \pm 1.04 $ & $ 8.15 \pm 0.20 $ & $ 23.75 \pm 1.49 $ & $ 41.11 \pm 1.46 $ & $ 54.85 \pm 1.40 $\\ 
& $\text{T}_{\text{Orig}} + \text{M}_{\text{Full}}$ & $ 27.22 \pm 1.30 $ & $ 40.19 \pm 1.01 $ & $ 35.67 \pm 0.48 $ & $ 20.80 \pm 0.56 $ & $ 27.04 \pm 1.74 $ & $ 61.43 \pm 1.14 $ & $ 78.10 \pm 1.31 $ & $ 1.98 \pm 0.10 $ & $ 26.56 \pm 1.55 $ & $ 49.67 \pm 1.60 $ & $ 52.88 \pm 1.40 $\\ 
& $\text{T}_{\text{PTP}} + \text{M}_{\text{Baseline}}$ & $ 25.34 \pm 1.27 $ & $ 41.29 \pm 1.01 $ & $ 35.79 \pm 0.48 $ & $ 22.40 \pm 0.57 $ & $ 26.57 \pm 1.73 $ & $ 61.81 \pm 1.13 $ & $ 76.60 \pm 1.34 $ & $ 2.32 \pm 0.11 $ & $ 24.72 \pm 1.51 $ & $ 48.85 \pm 1.60 $ & $ 52.96 \pm 1.40 $\\ 
& $\text{T}_{\text{Orig}} + \text{M}_{\text{Lex}}$ & $ 25.26 \pm 1.27 $ & $ 39.77 \pm 1.00 $ & $ 33.63 \pm 0.47 $ & $ 19.77 \pm 0.55 $ & $ 27.80 \pm 1.76 $ & $ 58.71 \pm 1.15 $ & $ 77.40 \pm 1.32 $ & $ 1.45 \pm 0.09 $ & $ 27.29 \pm 1.56 $ & $ 50.35 \pm 1.63 $ & $ 51.46 \pm 1.40 $\\ 
& $\text{T}_{\text{PTP}} + \text{M}_{\text{Lex}}$ & $ 27.39 \pm 1.30 $ & $ 40.11 \pm 1.01 $ & $ 33.84 \pm 0.47 $ & $ 19.38 \pm 0.55 $ & $ 27.50 \pm 1.75 $ & $ 57.29 \pm 1.15 $ & $ 77.50 \pm 1.32 $ & $ 0.95 \pm 0.07 $ & $ 26.68 \pm 1.55 $ & $ 49.90 \pm 1.63 $ & $ 51.46 \pm 1.40 $\\ 
\midrule 
\multirow[t]{5}{*}{1.4b}& Baseline & $ 32.17 \pm 1.37 $ & $ 62.67 \pm 0.99 $ & $ 54.92 \pm 0.50 $ & $ 49.33 \pm 0.69 $ & $ 22.89 \pm 1.65 $ & $ 71.87 \pm 1.05 $ & $ 92.40 \pm 0.84 $ & $ 19.39 \pm 0.30 $ & $ 22.89 \pm 1.47 $ & $ 38.68 \pm 1.40 $ & $ 56.43 \pm 1.39 $\\ 
& $\text{T}_{\text{Orig}} + \text{M}_{\text{Full}}$ & $ 26.19 \pm 1.28 $ & $ 37.33 \pm 0.99 $ & $ 33.29 \pm 0.47 $ & $ 17.90 \pm 0.53 $ & $ 27.34 \pm 1.75 $ & $ 56.96 \pm 1.16 $ & $ 65.30 \pm 1.51 $ & $ 2.56 \pm 0.12 $ & $ 26.93 \pm 1.55 $ & $ 52.00 \pm 1.61 $ & $ 53.75 \pm 1.40 $\\ 
& $\text{T}_{\text{PTP}} + \text{M}_{\text{Baseline}}$ & $ 24.91 \pm 1.26 $ & $ 38.59 \pm 1.00 $ & $ 33.07 \pm 0.47 $ & $ 15.60 \pm 0.50 $ & $ 26.88 \pm 1.74 $ & $ 56.64 \pm 1.16 $ & $ 65.40 \pm 1.51 $ & $ 2.36 \pm 0.11 $ & $ 26.19 \pm 1.54 $ & $ 51.00 \pm 1.61 $ & $ 53.99 \pm 1.40 $\\ 
& $\text{T}_{\text{Orig}} + \text{M}_{\text{Lex}}$ & $ 30.03 \pm 1.34 $ & $ 39.27 \pm 1.00 $ & $ 36.09 \pm 0.48 $ & $ 19.19 \pm 0.54 $ & $ 28.73 \pm 1.77 $ & $ 56.42 \pm 1.16 $ & $ 75.90 \pm 1.35 $ & $ 2.37 \pm 0.11 $ & $ 31.21 \pm 1.62 $ & $ 52.69 \pm 1.62 $ & $ 52.72 \pm 1.40 $\\ 
& $\text{T}_{\text{PTP}} + \text{M}_{\text{Lex}}$ & $ 28.75 \pm 1.32 $ & $ 40.99 \pm 1.01 $ & $ 37.21 \pm 0.48 $ & $ 19.73 \pm 0.55 $ & $ 28.57 \pm 1.77 $ & $ 55.98 \pm 1.16 $ & $ 74.80 \pm 1.37 $ & $ 3.12 \pm 0.13 $ & $ 30.23 \pm 1.61 $ & $ 52.49 \pm 1.65 $ & $ 52.72 \pm 1.40 $\\ 
% \midrule 
\bottomrule
\end{tabular}
\label{tbl:downstream}
\end{table*}

==> tables/test_col_70m_exp.tex <==
\begin{table}
\centering
\caption{table}
\label{tbl:70m_model_comparison}
\begin{tabular}{ccccc!{\vrule width \lightrulewidth}c} 
\toprule
\multicolumn{2}{c}{\textbf{Model}}                                        & \multicolumn{1}{l}{\graytext{$\text{T}_{\text{Orig}} + \text{M}_{\text{Baseline}}$}} & \multicolumn{1}{l}{$\text{T}_\text{Orig} + \text{M}_\text{Full}$} & \multicolumn{1}{l}{$\text{T}_\text{Orig} + \text{M}_\text{Lex}$} & \multicolumn{1}{l!{\vrule width \lightrulewidth}}{$\text{T}_\text{PTP} + \text{M}_\text{Full}$} & \multicolumn{1}{l}{$\text{T}_\text{PTP} + \text{M}_\text{Lex}$}  \\ 
\midrule
\multirow{3}{*}{\textbf{Pronoun Consistency ($\uparrow$)}} & \textbf{He}  & \graytext{96.82\textsubscript{0.79}}                                                 & 89.64\textsubscript{1.36}                                         & 86.46\textsubscript{1.54}                                        & 94.77\textsubscript{1.00}                                                                       & 84.97\textsubscript{1.56}                                        \\
                                                           & \textbf{She} & \graytext{71.59\textsubscript{2.00}}                                                 & 86.05\textsubscript{1.51}                                         & 72.87\textsubscript{1.97}                                        & 83.49\textsubscript{1.64}                                                                       & 72.21\textsubscript{1.95}                                        \\
                                                           & \textbf{Xe}  & \graytext{0.67\textsubscript{0.36}}                                                  & 14.46\textsubscript{1.56}                                         & 16.77\textsubscript{1.67}                                        & 37.79\textsubscript{2.15}                                                                       & 53.59\textsubscript{2.18}                                        \\ 
\hline\hline
\multirow{3}{*}{\textbf{Case Agreement ($\uparrow$)}}      & \textbf{He}  & \graytext{67.69\textsubscript{2.10}}                                                 & 68.51\textsubscript{2.08}                                         & 61.74\textsubscript{2.15}                                        & 69.49\textsubscript{2.03}                                                                       & 63.23\textsubscript{2.18}                                        \\
                                                           & \textbf{She} & \graytext{60.72\textsubscript{2.15}}                                                 & 59.69\textsubscript{2.21}                                         & 57.18\textsubscript{2.18}                                        & 61.08\textsubscript{2.18}                                                                       & 59.13\textsubscript{2.21}                                        \\
                                                           & \textbf{Xe}  & \graytext{20.00\textsubscript{1.77}}                                                 & 20.00\textsubscript{1.77}                                         & 20.00\textsubscript{1.74}                                        & 29.38\textsubscript{2.05}                                                                       & 32.51\textsubscript{2.08}                                        \\ 
\hline\hline
\multirow{3}{*}{\textbf{Error ($\downarrow$)}}             & \textbf{He}  & \graytext{23.85\textsubscript{1.90}}                                                 & 23.95\textsubscript{1.87}                                         & 28.97\textsubscript{1.97}                                        & 27.79\textsubscript{1.97}                                                                       & 25.79\textsubscript{1.92}                                        \\
                                                           & \textbf{She} & \graytext{16.92\textsubscript{1.67}}                                                 & 16.77\textsubscript{1.64}                                         & 23.18\textsubscript{1.87}                                        & 20.97\textsubscript{1.77}                                                                       & 21.85\textsubscript{1.82}                                        \\
                                                           & \textbf{Xe}  & \graytext{85.03\textsubscript{1.62}}                                                 & 89.49\textsubscript{1.38}                                         & 65.44\textsubscript{2.10}                                        & 27.03\textsubscript{1.97}                                                                       & 34.77\textsubscript{2.13}                                        \\
\bottomrule
\end{tabular}
\end{table}
